Towards Objective and Unbiased Decision Assessments with LLM-Enhanced Hierarchical Attention Networks

How objective and unbiased are we while making decisions? This work investigates cognitive bias identification in high-stake decision making process by human experts, questioning its effectiveness in real-world settings, such as candidates assessments for university admission. We begin with a statistical analysis assessing correlations among different decision points among in the current process, which discovers discrepancies that imply cognitive bias and inconsistency in decisions. This motivates our exploration of bias-aware AI-augmented workflow that surpass human judgment. We propose BGM-HAN, an enhanced Hierarchical Attention Network with Byte-Pair Encoding, Gated Residual Connections and Multi-Head Attention. Using it as a backbone model, we further propose a Shortlist-Analyse-Recommend (SAR) agentic workflow, which simulate real-world decision-making. In our experiments, both the proposed model and the agentic workflow significantly improves on both human judgment and alternative models, validated with real-world data.

==> sections/ack.tex <==
\section{Acknowledgement}

==> sections/futurework.tex <==
- add learnable weights to the features (profiles, analysis, shortlisting opinions). analyse the effect of the weights to the final recommendation outcome and its real-world implications
- Analysis with RA
- Further Ablation
- Data augmentation / create synthetic data for such data-limited scenarios to boost performance
- Investigate actual bias introduced by the interviews and human assessments

